Make It So: Steering StyleGAN for Any Image Inversion and Editing

StyleGAN's disentangled style representation enables powerful image editing by manipulating the latent variables, but accurately mapping real-world images to their latent variables (GAN inversion) remains a challenge. Existing GAN inversion methods struggle to maintain editing directions and produce realistic results. To address these limitations, we propose Make It So, a novel GAN inversion method that operates in the $\mathcal{Z}$ (noise) space rather than the typical $\mathcal{W}$ (latent style) space. Make It So preserves editing capabilities, even for out-of-domain images. This is a crucial property that was overlooked in prior methods. Our quantitative evaluations demonstrate that Make It So outperforms the state-of-the-art method PTI~\cite{roich2021pivotal} by a factor of five in inversion accuracy and achieves ten times better edit quality for complex indoor scenes.

==> fig_tex/face_stylespace.tex <==
\vspace{-5pt}
\begin{figure}[htpb!]
		\setlength{\linewidth}{\linewidth}
		\setlength{\hsize}{\linewidth}
		\centering
    \setlength\tabcolsep{0.5pt}
    \renewcommand{\arraystretch}{0.2}
    {
    \small
    \begin{tabular}{ccccccc}
		    \includegraphics[width=0.135\linewidth]{figures_supp/face_stylespace1/face1.jpg}
		    &
		    \includegraphics[width=0.135\linewidth]{figures_supp/face_stylespace1/inv.png} &
		     \includegraphics[width=0.135\linewidth]{figures_supp/face_stylespace1/smile1.jpg}
		    &
            \includegraphics[width=0.135\linewidth]{figures_supp/face_stylespace1/smile2.jpg}
		    &
		     \includegraphics[width=0.135\linewidth]{figures_supp/face_stylespace1/lip.jpg}
		    &
             \includegraphics[width=0.135\linewidth]{figures_supp/face_stylespace1/hair.jpg}
		    %
		    %
		    &
		    \includegraphics[width=0.135\linewidth]{figures_supp/face_stylespace1/dark.jpg}
		
		    %
		   	%
		    %
		    %
		    %
		    %
		    %
		    %
		    %
		    %
		    %
		    %
		      


		    \\

            \scriptsize{Target}& 
            \scriptsize{Inverted}&
            \scriptsize{Smile1}&
            \scriptsize{Smile2}&
            \scriptsize{Lipstick}&
            \scriptsize{Hairstyle}&
            \scriptsize{Hair color}
            \vspace{5pt}
            \\
        \end{tabular}
\vspace{-14pt}
\caption{ Additional face examples when using StyleSpace edits. %
}
\label{fig:rebfacess}
}

\end{figure}
